RePBubLik: Reducing the Polarized Bubble Radius with Link Insertions

The topology of the hyperlink graph among pages expressing different opinions may influence the exposure of readers to diverse content. Structural bias may trap a reader in a polarized bubble with no access to other opinions. We model readers' behavior as random walks. A node is in a polarized bubble if the expected length of a random walk from it to a page of different opinion is large. The structural bias of a graph is the sum of the radii of highly-polarized bubbles. We study the problem of decreasing the structural bias through edge insertions. Healing all nodes with high polarized bubble radius is hard to approximate within a logarithmic factor, so we focus on finding the best $k$ edges to insert to maximally reduce the structural bias. We present RePBubLik, an algorithm that leverages a variant of the random walk closeness centrality to select the edges to insert. RePBubLik obtains, under mild conditions, a constant-factor approximation. It reduces the structural bias faster than existing edge-recommendation methods, including some designed to reduce the polarization of a graph.

==> biblio.tex <==
%%% -*-BibTeX-*-
%%% Do NOT edit. File created by BibTeX with style
%%% ACM-Reference-Format-Journals [18-Jan-2012].

\begin{thebibliography}{62}

%%% ====================================================================
%%% NOTE TO THE USER: you can override these defaults by providing
%%% customized versions of any of these macros before the \bibliography
%%% command.  Each of them MUST provide its own final punctuation,
%%% except for \shownote{}, \showDOI{}, and \showURL{}.  The latter two
%%% do not use final punctuation, in order to avoid confusing it with
%%% the Web address.
%%%
%%% To suppress output of a particular field, define its macro to expand
%%% to an empty string, or better, \unskip, like this:
%%%
%%% \newcommand{\showDOI}[1]{\unskip}   % LaTeX syntax
%%%
%%% \def \showDOI #1{\unskip}           % plain TeX syntax
%%%
%%% ====================================================================

\ifx \showCODEN    \undefined \def \showCODEN     #1{\unskip}     \fi
\ifx \showDOI      \undefined \def \showDOI       #1{#1}\fi
\ifx \showISBNx    \undefined \def \showISBNx     #1{\unskip}     \fi
\ifx \showISBNxiii \undefined \def \showISBNxiii  #1{\unskip}     \fi
\ifx \showISSN     \undefined \def \showISSN      #1{\unskip}     \fi
\ifx \showLCCN     \undefined \def \showLCCN      #1{\unskip}     \fi
\ifx \shownote     \undefined \def \shownote      #1{#1}          \fi
\ifx \showarticletitle \undefined \def \showarticletitle #1{#1}   \fi
\ifx \showURL      \undefined \def \showURL       {\relax}        \fi
% The following commands are used for tagged output and should be
% invisible to TeX
\providecommand\bibfield[2]{#2}
\providecommand\bibinfo[2]{#2}
\providecommand\natexlab[1]{#1}
\providecommand\showeprint[2][]{arXiv:#2}



\bibitem[\protect\citeauthoryear{Bera and Seshadhri}{Bera and Seshadhri}{2020}]%
        {Bera2020}
\bibfield{author}{\bibinfo{person}{Suman K. Bera} {and}
  \bibinfo{person}{C Seshadhri}.} \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{How to Count Triangles, without Seeing the Whole Graph}. 
. In Proceedings of the 26th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining.
\newblock

\bibitem[\protect\citeauthoryear{ Chierichetti,  Dasgupta, Kumar,  Lattanzi, and  Sarlos}{Chierichetti et~al\mbox{.}}{2016}]%
        {WWW2016Chierichetti}
\bibfield{author}{\bibinfo{person}{Flavio Chierichetti} {and}
  \bibinfo{person}{Anirban Dasgupta} {and}
  \bibinfo{person}{Ravi Kumar}{and}
  \bibinfo{person}{Silvio Lattanzi}{and}
  \bibinfo{person}{Tamas Sarlos}.} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{On
sampling nodes in a network}. 
. In Proceedings of the 25th International Conference on World
Wide Web, WWW '16).
\newblock


\bibitem[\protect\citeauthoryear{Chierichetti and Haddadan}{Chierichetti and Haddadan}{2018}]%
        {HaddadanIcalp2018}
\bibfield{author}{\bibinfo{person}{Flavio Chierichetti} {and}
  \bibinfo{person}{Shahrzad Haddadan}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{On the Complexity of Sampling Vertices Uniformly from a Graph}. 
45th International Colloquium on Automata, Languages, and Programming (ICALP 2018).
\newblock


\bibitem[\protect\citeauthoryear{Ben-Hamou, Anna and Oliveira, Roberto I. and Peres, Yuval}{Ben-Hamou et~al\mbox{.}}{2018}]%
        {peresSODA2018}
\bibfield{author}{\bibinfo{person}{Anna Ben-Hamou} {and}
  \bibinfo{person}{Roberto Oliveira}  {and}
  \bibinfo{person}{Yuval Peres}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Estimating Graph Parameters via Random Walks with Restarts}. SODA'18, Proceedings of the Twenty-Ninth Annual ACM-SIAM Symposium on Discrete Algorithms.
\newblock



\bibitem[\protect\citeauthoryear{Adamic and Glance}{Adamic and Glance}{2005}]%
        {adamic2005political}
\bibfield{author}{\bibinfo{person}{Lada~A Adamic} {and}
  \bibinfo{person}{Natalie Glance}.} \bibinfo{year}{2005}\natexlab{}.
\newblock \showarticletitle{The political blogosphere and the 2004 US election:
  divided they blog}. WWW'05 Workshop on Weblogging Ecosystem.
\newblock


\bibitem[\protect\citeauthoryear{Akoglu}{Akoglu}{2014}]%
        {Akoglu14}
\bibfield{author}{\bibinfo{person}{Leman Akoglu}.}
  \bibinfo{year}{2014}\natexlab{}.
\newblock \showarticletitle{Quantifying political polarity based on bipartite
  opinion networks}. AAA'14.
\newblock


\bibitem[\protect\citeauthoryear{Anagnostopoulos, Becchetti, Fazzone, Menghini,
  and Schwiegelshohn}{Anagnostopoulos et~al\mbox{.}}{2019}]%
        {anagnostopoulos2019principal}
\bibfield{author}{\bibinfo{person}{Aris Anagnostopoulos}, \bibinfo{person}{Luca
  Becchetti}, \bibinfo{person}{Adriano Fazzone}, \bibinfo{person}{Cristina
  Menghini}, {and} \bibinfo{person}{Chris Schwiegelshohn}.}
  \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Principal fairness: removing bias via projections}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:1905.13651}}
  (\bibinfo{year}{2019}).
\newblock


\bibitem[\protect\citeauthoryear{Angriman, van~der Grinten, Bojchevski,
  Z{\"u}gner, G{\"u}nnemann, and Meyerhenke}{Angriman et~al\mbox{.}}{2020}]%
        {angriman2020group}
\bibfield{author}{\bibinfo{person}{Eugenio Angriman},
  \bibinfo{person}{Alexander van~der Grinten}, \bibinfo{person}{Aleksandar
  Bojchevski}, \bibinfo{person}{Daniel Z{\"u}gner}, \bibinfo{person}{Stephan
  G{\"u}nnemann}, {and} \bibinfo{person}{Henning Meyerhenke}.}
  \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{Group Centrality Maximization for Large-scale
  Graphs}. In ALENEX'20.
\newblock


\bibitem[\protect\citeauthoryear{Arrigo and Benzi}{Arrigo and Benzi}{2016a}]%
        {arrigo2016edge}
\bibfield{author}{\bibinfo{person}{Francesca Arrigo} {and}
  \bibinfo{person}{Michele Benzi}.} \bibinfo{year}{2016}\natexlab{a}.
\newblock \showarticletitle{Edge modification criteria for enhancing the
  communicability of digraphs}.
\newblock \bibinfo{journal}{\emph{SIAM J. Matrix Anal. Appl.}}
  \bibinfo{volume}{37} (\bibinfo{year}{2016}).
\newblock


\bibitem[\protect\citeauthoryear{Arrigo and Benzi}{Arrigo and Benzi}{2016b}]%
        {arrigo2016updating}
\bibfield{author}{\bibinfo{person}{Francesca Arrigo} {and}
  \bibinfo{person}{Michele Benzi}.} \bibinfo{year}{2016}\natexlab{b}.
\newblock \showarticletitle{Updating and downdating techniques for optimizing
  network communicability}.
\newblock \bibinfo{journal}{\emph{SIAM J. Sci. Comp.}}
  \bibinfo{volume}{38}, \bibinfo{number}{1} (\bibinfo{year}{2016})
\newblock


\bibitem[\protect\citeauthoryear{Aslay, Matakos, Galbrun, and Gionis}{Aslay
  et~al\mbox{.}}{2018}]%
        {AslayMGG18}
\bibfield{author}{\bibinfo{person}{Cigdem Aslay}, \bibinfo{person}{Antonis
  Matakos}, \bibinfo{person}{Esther Galbrun}, {and} \bibinfo{person}{Aristides
  Gionis}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Maximizing the Diversity of Exposure in a Social
  Network}. ICDM'18.
\newblock


\bibitem[\protect\citeauthoryear{Bakshy, Messing, and Adamic}{Bakshy
  et~al\mbox{.}}{2015}]%
        {bakshy2015exposure}
\bibfield{author}{\bibinfo{person}{Eytan Bakshy}, \bibinfo{person}{Solomon
  Messing}, {and} \bibinfo{person}{Lada~A Adamic}.}
  \bibinfo{year}{2015}\natexlab{}.
\newblock \showarticletitle{Exposure to ideologically diverse news and opinion
  on Facebook}.
\newblock \bibinfo{journal}{\emph{Science}} \bibinfo{volume}{348},
  \bibinfo{number}{6239} (\bibinfo{year}{2015}), \bibinfo{pages}{1130--1132}.
\newblock


\bibitem[\protect\citeauthoryear{Becker, Cor{\`o}, D'Angelo, and
  Gilbert}{Becker et~al\mbox{.}}{2020}]%
        {BeckerCDAG20}
\bibfield{author}{\bibinfo{person}{Ruben Becker}, \bibinfo{person}{Federico
  Cor{\`o}}, \bibinfo{person}{Gianlorenzo D'Angelo}, {and}
  \bibinfo{person}{Hugo Gilbert}.} \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{Balancing Spreads of Influence in a Social
  Network}.
\newblock AAAI'20.
\newblock


\bibitem[\protect\citeauthoryear{Benhabib}{Benhabib}{1996}]%
        {benhabib1996toward}
\bibfield{author}{\bibinfo{person}{Seyla Benhabib}.}
  \bibinfo{year}{1996}\natexlab{}.
\newblock \showarticletitle{Toward a deliberative model of democratic
  legitimacy}.
\newblock \bibinfo{journal}{\emph{Democracy and difference: Contesting the
  boundaries of the political}} (\bibinfo{year}{1996}),
  \bibinfo{pages}{67--94}.
\newblock


\bibitem[\protect\citeauthoryear{Bergamini, Crescenzi, D'angelo, Meyerhenke,
  Severini, and Velaj}{Bergamini et~al\mbox{.}}{2018}]%
        {bergamini2018improving}
\bibfield{author}{\bibinfo{person}{Elisabetta Bergamini},
  \bibinfo{person}{Pierluigi Crescenzi}, \bibinfo{person}{Gianlorenzo
  D'angelo}, \bibinfo{person}{Henning Meyerhenke}, \bibinfo{person}{Lorenzo
  Severini}, {and} \bibinfo{person}{Yllka Velaj}.}
  \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Improving the betweenness centrality of a node by
  adding links}.
\newblock \bibinfo{journal}{\emph{J.~Exper.~Algo. (JEA)}}
  \bibinfo{volume}{23} (\bibinfo{year}{2018}), \bibinfo{pages}{1--32}.
\newblock


\bibitem[\protect\citeauthoryear{Chan, Akoglu, and Tong}{Chan
  et~al\mbox{.}}{2014}]%
        {chan2014make}
\bibfield{author}{\bibinfo{person}{Hau Chan}, \bibinfo{person}{Leman Akoglu},
  {and} \bibinfo{person}{Hanghang Tong}.} \bibinfo{year}{2014}\natexlab{}.
\newblock \showarticletitle{Make it or break it: Manipulating robustness in
  large networks}. In SDM'14.
\newblock


\bibitem[\protect\citeauthoryear{Chitra and Musco}{Chitra and Musco}{2020}]%
        {ChitraM20}
\bibfield{author}{\bibinfo{person}{Uthsav Chitra} {and}
  \bibinfo{person}{Christopher Musco}.} \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{Analyzing the Impact of Filter Bubbles on Social
  Network Polarization}. WSDM'20.
\newblock


\bibitem[\protect\citeauthoryear{Conover, Ratkiewicz, Francisco,
  Gon{\c{c}}alves, Menczer, and Flammini}{Conover et~al\mbox{.}}{2011}]%
        {conover2011political}
\bibfield{author}{\bibinfo{person}{Michael~D Conover}, \bibinfo{person}{Jacob
  Ratkiewicz}, \bibinfo{person}{Matthew Francisco}, \bibinfo{person}{Bruno
  Gon{\c{c}}alves}, \bibinfo{person}{Filippo Menczer}, {and}
  \bibinfo{person}{Alessandro Flammini}.} \bibinfo{year}{2011}\natexlab{}.
\newblock \showarticletitle{Political polarization on twitter}. ICWSM'11.
\newblock


\bibitem[\protect\citeauthoryear{Cossard, De~Francisci~Morales, Kalimeri,
  Mejova, Paolotti, and Starnini}{Cossard et~al\mbox{.}}{2020}]%
        {CossardDFMKMPS20}
\bibfield{author}{\bibinfo{person}{Alessandro Cossard},
  \bibinfo{person}{Gianmarco De~Francisci~Morales}, \bibinfo{person}{Kyriaki
  Kalimeri}, \bibinfo{person}{Yelena Mejova}, \bibinfo{person}{Daniela
  Paolotti}, {and} \bibinfo{person}{Michele Starnini}.}
  \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{Falling into the Echo Chamber: The {I}talian
  Vaccination Debate on {T}witter}. ICWSM'20.
\newblock


\bibitem[\protect\citeauthoryear{D'Angelo, Olsen, and Severini}{D'Angelo
  et~al\mbox{.}}{2019}]%
        {d2019coverage}
\bibfield{author}{\bibinfo{person}{Gianlorenzo D'Angelo},
  \bibinfo{person}{Martin Olsen}, {and} \bibinfo{person}{Lorenzo Severini}.}
  \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Coverage centrality maximization in undirected
  networks}. AAA'19.
\newblock


\bibitem[\protect\citeauthoryear{Das, Gollapudi, and Munagala}{Das
  et~al\mbox{.}}{2014}]%
        {DasGM14}
\bibfield{author}{\bibinfo{person}{Abhimanyu Das}, \bibinfo{person}{Sreenivas
  Gollapudi}, {and} \bibinfo{person}{Kamesh Munagala}.}
  \bibinfo{year}{2014}\natexlab{}.
\newblock \showarticletitle{Modeling opinion dynamics in social networks}. WSDM'14.
\newblock


\bibitem[\protect\citeauthoryear{Demaine and Zadimoghaddam}{Demaine and
  Zadimoghaddam}{2010}]%
        {demaine2010minimizing}
\bibfield{author}{\bibinfo{person}{Erik~D Demaine} {and}
  \bibinfo{person}{Morteza Zadimoghaddam}.} \bibinfo{year}{2010}\natexlab{}.
\newblock \showarticletitle{Minimizing the diameter of a network using shortcut
  edges}. SWAT'10.
\newblock


\bibitem[\protect\citeauthoryear{Dumitriu, Tetali, and Winkler}{Dumitriu
  et~al\mbox{.}}{2003}]%
        {rwwithrestart}
\bibfield{author}{\bibinfo{person}{Ioana Dumitriu}, \bibinfo{person}{Prasad
  Tetali}, {and} \bibinfo{person}{Peter Winkler}.}
  \bibinfo{year}{2003}\natexlab{}.
\newblock \showarticletitle{On Playing Golf with Two Balls}.
\newblock \bibinfo{journal}{\emph{SIAM J. Discrete Math.}}
  \bibinfo{volume}{16} (\bibinfo{year}{2003}), \bibinfo{pages}{604--615}.
\newblock


\bibitem[\protect\citeauthoryear{Fagin, Karlin, Kleinberg, Raghavan,
  Rajagopalan, Rubinfeld, and Tomkins}{Fagin et~al\mbox{.}}{2001}]%
        {rwwithbackbutton}
\bibfield{author}{\bibinfo{person}{Ronald Fagin}, \bibinfo{person}{Anna
  Karlin}, \bibinfo{person}{Jon Kleinberg}, \bibinfo{person}{Prabhakar
  Raghavan}, \bibinfo{person}{Sridhar Rajagopalan}, \bibinfo{person}{Ronitt
  Rubinfeld}, {and} \bibinfo{person}{Andrew Tomkins}.}
  \bibinfo{year}{2001}\natexlab{}.
\newblock \showarticletitle{Random Walks with "Back Buttons"}.
\newblock \bibinfo{journal}{\emph{The Annals of Applied Probability}}
  \bibinfo{volume}{11} (\bibinfo{date}{06} \bibinfo{year}{2001}).
\newblock


\bibitem[\protect\citeauthoryear{Flaxman, Goel, and Rao}{Flaxman
  et~al\mbox{.}}{2016}]%
        {flaxman2016filter}
\bibfield{author}{\bibinfo{person}{Seth Flaxman}, \bibinfo{person}{Sharad
  Goel}, {and} \bibinfo{person}{Justin~M Rao}.}
  \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{Filter bubbles, echo chambers, and online news
  consumption}.
\newblock \bibinfo{journal}{\emph{Public opinion quarterly}}
  \bibinfo{volume}{80}, \bibinfo{number}{S1} (\bibinfo{year}{2016}),
  \bibinfo{pages}{298--320}.
\newblock


\bibitem[\protect\citeauthoryear{Garimella, De~Francisci~Morales, Gionis, and
  Mathioudakis}{Garimella et~al\mbox{.}}{2017a}]%
        {garimella2017reducing}
\bibfield{author}{\bibinfo{person}{Kiran Garimella}, \bibinfo{person}{Gianmarco
  De~Francisci~Morales}, \bibinfo{person}{Aristides Gionis}, {and}
  \bibinfo{person}{Michael Mathioudakis}.} \bibinfo{year}{2017}\natexlab{a}.
\newblock \showarticletitle{Reducing Controversy by Connecting Opposing Views}.
  WSDM'17.
\newblock


\bibitem[\protect\citeauthoryear{Garimella, De~Francisci~Morales, Gionis, and
  Mathioudakis}{Garimella et~al\mbox{.}}{2018a}]%
        {GarimellaDFMGM18}
\bibfield{author}{\bibinfo{person}{Kiran Garimella}, \bibinfo{person}{Gianmarco
  De~Francisci~Morales}, \bibinfo{person}{Aristides Gionis}, {and}
  \bibinfo{person}{Michael Mathioudakis}.} \bibinfo{year}{2018}\natexlab{a}.
\newblock \showarticletitle{Political discourse on social media: Echo chambers,
  gatekeepers, and the price of bipartisanship}. WWW'18.
\newblock


\bibitem[\protect\citeauthoryear{Garimella, Gionis, Parotsidis, and
  Tatti}{Garimella et~al\mbox{.}}{2017b}]%
        {GarimellaGPT17}
\bibfield{author}{\bibinfo{person}{Kiran Garimella}, \bibinfo{person}{Aristides
  Gionis}, \bibinfo{person}{Nikos Parotsidis}, {and} \bibinfo{person}{Nikolaj
  Tatti}.} \bibinfo{year}{2017}\natexlab{b}.
\newblock \showarticletitle{Balancing information exposure in social networks}.
  NeurIPS'17.
\newblock


\bibitem[\protect\citeauthoryear{Garimella, Morales, Gionis, and
  Mathioudakis}{Garimella et~al\mbox{.}}{2018b}]%
        {garimella2018quantifying}
\bibfield{author}{\bibinfo{person}{Kiran Garimella}, \bibinfo{person}{Gianmarco
  De~Francisci Morales}, \bibinfo{person}{Aristides Gionis}, {and}
  \bibinfo{person}{Michael Mathioudakis}.} \bibinfo{year}{2018}\natexlab{b}.
\newblock \showarticletitle{Quantifying controversy on social media}.
\newblock \bibinfo{journal}{\emph{ACM Trans. Soc. Comp.}}
  (\bibinfo{year}{2018}).
\newblock


\bibitem[\protect\citeauthoryear{Ge, Delgado-Battenfeld, and Jannach}{Ge
  et~al\mbox{.}}{2010}]%
        {mouzhi2010serendipity}
\bibfield{author}{\bibinfo{person}{Mouzhi Ge}, \bibinfo{person}{Carla
  Delgado-Battenfeld}, {and} \bibinfo{person}{Dietmar Jannach}.}
  \bibinfo{year}{2010}\natexlab{}.
\newblock \showarticletitle{Beyond Accuracy: Evaluating Recommender Systems by
  Coverage and Serendipity}. RecSys'10.
\newblock


\bibitem[\protect\citeauthoryear{Grover and Leskovec}{Grover and
  Leskovec}{2016}]%
        {grover2016node2vec}
\bibfield{author}{\bibinfo{person}{Aditya Grover} {and} \bibinfo{person}{Jure
  Leskovec}.} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{node2vec: Scalable feature learning for networks}.
  In \bibinfo{booktitle}{\emph{Proceedings of the 22nd ACM SIGKDD international
  conference on Knowledge discovery and data mining}}.
  \bibinfo{pages}{855--864}.
\newblock


\bibitem[\protect\citeauthoryear{Guerra, Meira~Jr, Cardie, and
  Kleinberg}{Guerra et~al\mbox{.}}{2013}]%
        {guerra2013measure}
\bibfield{author}{\bibinfo{person}{Pedro~Calais Guerra},
  \bibinfo{person}{Wagner Meira~Jr}, \bibinfo{person}{Claire Cardie}, {and}
  \bibinfo{person}{Robert Kleinberg}.} \bibinfo{year}{2013}\natexlab{}.
\newblock \showarticletitle{A measure of polarization on social media networks
  based on community boundaries}. In \bibinfo{booktitle}{\emph{Seventh
  International AAAI Conference on Weblogs and Social Media}}.
\newblock


\bibitem[\protect\citeauthoryear{Isenberg}{Isenberg}{1986}]%
        {Isenberg86}
\bibfield{author}{\bibinfo{person}{Daniel~J. Isenberg}.}
  \bibinfo{year}{1986}\natexlab{}.
\newblock \showarticletitle{Group polarization: A critical review and
  meta-analysis.}
\newblock \bibinfo{journal}{\emph{Journal of personality and social
  psychology}} \bibinfo{volume}{50}, \bibinfo{number}{6}
  (\bibinfo{year}{1986}), \bibinfo{pages}{1141}.
\newblock


\bibitem[\protect\citeauthoryear{Kotkov, Veijalainen, and Wang}{Kotkov
  et~al\mbox{.}}{2016}]%
        {kotkov2016chalserendipity}
\bibfield{author}{\bibinfo{person}{Denis Kotkov}, \bibinfo{person}{Jari
  Veijalainen}, {and} \bibinfo{person}{Shuaiqiang Wang}.}
  \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{Challenges of serendipity in recommender systems}.
  In \bibinfo{booktitle}{\emph{WEBIST 2016: Proceedings of the 12th
  International conference on web information systems and technologies.}}
\newblock


\bibitem[\protect\citeauthoryear{Kumar, Hamilton, Leskovec, and Jurafsky}{Kumar
  et~al\mbox{.}}{2018}]%
        {KumarHLJ18}
\bibfield{author}{\bibinfo{person}{Srijan Kumar}, \bibinfo{person}{William~L.
  Hamilton}, \bibinfo{person}{Jure Leskovec}, {and} \bibinfo{person}{Dan
  Jurafsky}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Community interaction and conflict on the web}. In
  \bibinfo{booktitle}{\emph{Proceedings of the 2018 World Wide Web
  Conference}}. \bibinfo{pages}{933--943}.
\newblock


\bibitem[\protect\citeauthoryear{LeFebvre}{LeFebvre}{2017}]%
        {LeFebvre17}
\bibfield{author}{\bibinfo{person}{Rob LeFebvre}.}
  \bibinfo{year}{2017}\natexlab{}.
\newblock \bibinfo{title}{{O}bama {F}oundation taps social media to fight
  online echo chambers}.  (\bibinfo{year}{2017}).
\newblock


\bibitem[\protect\citeauthoryear{Leskovec, Adamic, and Huberman}{Leskovec
  et~al\mbox{.}}{2007}]%
        {leskovec2007dynamics}
\bibfield{author}{\bibinfo{person}{Jure Leskovec}, \bibinfo{person}{Lada~A
  Adamic}, {and} \bibinfo{person}{Bernardo~A Huberman}.}
  \bibinfo{year}{2007}\natexlab{}.
\newblock \showarticletitle{The dynamics of viral marketing}.
\newblock \bibinfo{journal}{\emph{ACM Trans. on the Web (TWEB)}}
  \bibinfo{volume}{1}, \bibinfo{number}{1} (\bibinfo{year}{2007}),
  \bibinfo{pages}{5--es}.
\newblock


\bibitem[\protect\citeauthoryear{Liao and Fu}{Liao and Fu}{2014a}]%
        {LiaoF14a}
\bibfield{author}{\bibinfo{person}{Q~Vera Liao} {and} \bibinfo{person}{Wai-Tat
  Fu}.} \bibinfo{year}{2014}\natexlab{a}.
\newblock \showarticletitle{Can you hear me now? Mitigating the echo chamber
  effect by source position indicators}. In
  \bibinfo{booktitle}{\emph{Proceedings of the 17th ACM conference on Computer
  supported cooperative work \& social computing}}. \bibinfo{pages}{184--196}.
\newblock


\bibitem[\protect\citeauthoryear{Liao and Fu}{Liao and Fu}{2014b}]%
        {LiaoF14b}
\bibfield{author}{\bibinfo{person}{Q.~Vera Liao} {and} \bibinfo{person}{Wai-Tat
  Fu}.} \bibinfo{year}{2014}\natexlab{b}.
\newblock \showarticletitle{Expert voices in echo chambers: effects of source
  expertise indicators on exposure to diverse opinions}. CHI'14.
\newblock


\bibitem[\protect\citeauthoryear{Mahmoody, Tsourakakis, and Upfal}{Mahmoody
  et~al\mbox{.}}{2016}]%
        {mahmoody2016scalable}
\bibfield{author}{\bibinfo{person}{Ahmad Mahmoody},
  \bibinfo{person}{Charalampos~E Tsourakakis}, {and} \bibinfo{person}{Eli
  Upfal}.} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{Scalable betweenness centrality maximization via
  sampling}. KDD'16.
\newblock


\bibitem[\protect\citeauthoryear{Matakos, Terzi, and Tsaparas}{Matakos
  et~al\mbox{.}}{2017}]%
        {MakatosTT17}
\bibfield{author}{\bibinfo{person}{Antonis Matakos}, \bibinfo{person}{Evimaria
  Terzi}, {and} \bibinfo{person}{Panayiotis Tsaparas}.}
  \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{Measuring and moderating opinion polarization in
  social networks}.
\newblock \bibinfo{journal}{\emph{Data Mining and Knowledge Discovery}}
  \bibinfo{volume}{31} (\bibinfo{year}{2017}), \bibinfo{pages}{1480--1505}.
\newblock


\bibitem[\protect\citeauthoryear{Matakos, Tu, and Gionis}{Matakos
  et~al\mbox{.}}{2020}]%
        {MatakosTG20}
\bibfield{author}{\bibinfo{person}{Antonis Matakos}, \bibinfo{person}{Sijing
  Tu}, {and} \bibinfo{person}{Aristides Gionis}.}
  \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{Tell me something my friends do not know: diversity
  maximization in social networks}.
\newblock \bibinfo{journal}{\emph{Knowledge and Information Systems}}
  \bibinfo{number}{9} (\bibinfo{year}{2020}), \bibinfo{pages}{3697--3726}.
\newblock


\bibitem[\protect\citeauthoryear{Medya, Silva, Singh, Basu, and Swami}{Medya
  et~al\mbox{.}}{2018}]%
        {medya2018group}
\bibfield{author}{\bibinfo{person}{Sourav Medya}, \bibinfo{person}{Arlei
  Silva}, \bibinfo{person}{Ambuj Singh}, \bibinfo{person}{Prithwish Basu},
  {and} \bibinfo{person}{Ananthram Swami}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Group centrality maximization via network design}.
  SDM'18.
\newblock


\bibitem[\protect\citeauthoryear{Mejova, Zhang, Diakopoulos, and
  Castillo}{Mejova et~al\mbox{.}}{2014}]%
        {mejova2014controversy}
\bibfield{author}{\bibinfo{person}{Yelena Mejova}, \bibinfo{person}{Amy~X
  Zhang}, \bibinfo{person}{Nicholas Diakopoulos}, {and} \bibinfo{person}{Carlos
  Castillo}.} \bibinfo{year}{2014}\natexlab{}.
\newblock \showarticletitle{Controversy and sentiment in online news}.
\newblock \bibinfo{journal}{\emph{arXiv preprint}} (\bibinfo{year}{2014}).
\newblock


\bibitem[\protect\citeauthoryear{{Menghini}, {Anagnostopoulos}, and
  {Upfal}}{{Menghini} et~al\mbox{.}}{2019}]%
        {menghini2019wikipol}
\bibfield{author}{\bibinfo{person}{C. {Menghini}}, \bibinfo{person}{A.
  {Anagnostopoulos}}, {and} \bibinfo{person}{E. {Upfal}}.}
  \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Wikipedia Polarization and Its Effects on
  Navigation Paths}. BigData'19.
\newblock


\bibitem[\protect\citeauthoryear{Menghini, Anagnostopoulos, and Upfal}{Menghini
  et~al\mbox{.}}{2020}]%
        {menghini2020wikipedias}
\bibfield{author}{\bibinfo{person}{Cristina Menghini}, \bibinfo{person}{Aris
  Anagnostopoulos}, {and} \bibinfo{person}{Eli Upfal}.}
  \bibinfo{year}{2020}\natexlab{}.
\newblock \bibinfo{title}{Wikipedia's Network Bias on Controversial Topics}.
\newblock
\newblock
\urldef\tempurl%
\url{https://arxiv.org/abs/2007.08197}
\showURL{%
\tempurl}


\bibitem[\protect\citeauthoryear{Morales, Borondo, Losada, and Benito}{Morales
  et~al\mbox{.}}{2015}]%
        {MoralesBLB15}
\bibfield{author}{\bibinfo{person}{Alfredo~Jose Morales},
  \bibinfo{person}{Javier Borondo}, \bibinfo{person}{Juan~Carlos Losada}, {and}
  \bibinfo{person}{Rosa~M. Benito}.} \bibinfo{year}{2015}\natexlab{}.
\newblock \showarticletitle{Measuring political polarization: Twitter shows the
  two sides of Venezuela}.
\newblock \bibinfo{journal}{\emph{Chaos: An Interdisciplinary Journal of
  Nonlinear Science}} \bibinfo{volume}{25}, \bibinfo{number}{3}
  (\bibinfo{year}{2015}), \bibinfo{pages}{033114}.
\newblock


\bibitem[\protect\citeauthoryear{Mossel and Tamuz}{Mossel and Tamuz}{2017}]%
        {MosselT17}
\bibfield{author}{\bibinfo{person}{Elchanan Mossel} {and} \bibinfo{person}{Omer
  Tamuz}.} \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{Opinion exchange dynamics}.
\newblock \bibinfo{journal}{\emph{Probability Surveys}}  \bibinfo{volume}{14}
  (\bibinfo{year}{2017}), \bibinfo{pages}{155--204}.
\newblock


\bibitem[\protect\citeauthoryear{Munson, Lee, and Resnick}{Munson
  et~al\mbox{.}}{2013}]%
        {MunsonLR13}
\bibfield{author}{\bibinfo{person}{Sean~A Munson},
  \bibinfo{person}{Stephanie~Y. Lee}, {and} \bibinfo{person}{Paul Resnick}.}
  \bibinfo{year}{2013}\natexlab{}.
\newblock \showarticletitle{Encouraging reading of diverse political viewpoints
  with a browser widget}. ICWSM'13.
\newblock


\bibitem[\protect\citeauthoryear{Musco, Musco, and Tsourakakis}{Musco
  et~al\mbox{.}}{2018}]%
        {MuscoMT18}
\bibfield{author}{\bibinfo{person}{Cameron Musco}, \bibinfo{person}{Christopher
  Musco}, {and} \bibinfo{person}{Charalampos~E. Tsourakakis}.}
  \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Minimizing Polarization and Disagreement in Social
  Networks}. WWW'18.
\newblock


\bibitem[\protect\citeauthoryear{Nelimarkka, Laaksonen, and Semaan}{Nelimarkka
  et~al\mbox{.}}{2018}]%
        {NelimarkkaLS18}
\bibfield{author}{\bibinfo{person}{Matti Nelimarkka},
  \bibinfo{person}{Salla-Maaria Laaksonen}, {and} \bibinfo{person}{Bryan
  Semaan}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Social media is polarized, social media is
  polarized: towards a new design agenda for mitigating polarization}. In
  \bibinfo{booktitle}{\emph{Proceedings of the 2018 Designing Interactive
  Systems Conference}}. \bibinfo{pages}{957--970}.
\newblock


\bibitem[\protect\citeauthoryear{Papagelis, Bonchi, and Gionis}{Papagelis
  et~al\mbox{.}}{2011}]%
        {papagelis2011suggesting}
\bibfield{author}{\bibinfo{person}{Manos Papagelis}, \bibinfo{person}{Francesco
  Bonchi}, {and} \bibinfo{person}{Aristides Gionis}.}
  \bibinfo{year}{2011}\natexlab{}.
\newblock \showarticletitle{Suggesting ghost edges for a smaller world}. CIKM'11.
\newblock


\bibitem[\protect\citeauthoryear{Pariser}{Pariser}{2011}]%
        {Pariser11}
\bibfield{author}{\bibinfo{person}{Eli Pariser}.}
  \bibinfo{year}{2011}\natexlab{}.
\newblock \bibinfo{booktitle}{\emph{The filter bubble: What the {I}nternet is
  hiding from you}}.
\newblock \bibinfo{publisher}{Penguin}.
\newblock


\bibitem[\protect\citeauthoryear{Parotsidis, Pitoura, and Tsaparas}{Parotsidis
  et~al\mbox{.}}{2015}]%
        {parotsidis2015selecting}
\bibfield{author}{\bibinfo{person}{Nikos Parotsidis},
  \bibinfo{person}{Evaggelia Pitoura}, {and} \bibinfo{person}{Panayiotis
  Tsaparas}.} \bibinfo{year}{2015}\natexlab{}.
\newblock \showarticletitle{Selecting shortcuts for a smaller world}. SDM'15.
\newblock


\bibitem[\protect\citeauthoryear{Parotsidis, Pitoura, and Tsaparas}{Parotsidis
  et~al\mbox{.}}{2016}]%
        {parotsidis2016centrality}
\bibfield{author}{\bibinfo{person}{Nikos Parotsidis},
  \bibinfo{person}{Evaggelia Pitoura}, {and} \bibinfo{person}{Panayiotis
  Tsaparas}.} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{Centrality-aware link recommendations}. WSDM'16.
\newblock


\bibitem[\protect\citeauthoryear{Perumal, Basu, and Guan}{Perumal
  et~al\mbox{.}}{2013}]%
        {perumal2013minimizing}
\bibfield{author}{\bibinfo{person}{Senni Perumal}, \bibinfo{person}{Prithwish
  Basu}, {and} \bibinfo{person}{Ziyu Guan}.} \bibinfo{year}{2013}\natexlab{}.
\newblock \showarticletitle{Minimizing eccentricity in composite networks via
  constrained edge additions}. MILCOM'13.
\newblock


\bibitem[\protect\citeauthoryear{Rastegarpanah, Gummadi, and
  Crovella}{Rastegarpanah et~al\mbox{.}}{2019}]%
        {RastegarpahahGC2019}
\bibfield{author}{\bibinfo{person}{Bashir Rastegarpanah},
  \bibinfo{person}{Krishna~P. Gummadi}, {and} \bibinfo{person}{Mark Crovella}.}
  \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Fighting Fire with Fire: Using Antidote Data to
  Improve Polarization and Fairness of Recommender Systems}. WSDM'19.
\newblock


\bibitem[\protect\citeauthoryear{Ribeiro, Ottoni, West, Almeida, and
  Meira}{Ribeiro et~al\mbox{.}}{2020}]%
        {horta2020youtube}
\bibfield{author}{\bibinfo{person}{Manoel~Horta Ribeiro},
  \bibinfo{person}{Raphael Ottoni}, \bibinfo{person}{Robert West},
  \bibinfo{person}{Virg\'{\i}lio A.~F. Almeida}, {and} \bibinfo{person}{Wagner
  Meira}.} \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{Auditing Radicalization Pathways on YouTube}. FAT'20.
\newblock


\bibitem[\protect\citeauthoryear{Stoica and Chaintreau}{Stoica and
  Chaintreau}{2019}]%
        {StoicaC19}
\bibfield{author}{\bibinfo{person}{Ana-Andreea Stoica} {and}
  \bibinfo{person}{Augustin Chaintreau}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Hegemony in Social Media and the effect of
  recommendations}.
\newblock WWW'19.
\newblock


\bibitem[\protect\citeauthoryear{Stoica, Han, and Chaintreau}{Stoica
  et~al\mbox{.}}{2020}]%
        {StoicaHC20}
\bibfield{author}{\bibinfo{person}{Ana-Andreea Stoica},
  \bibinfo{person}{Jessy~Xinyi Han}, {and} \bibinfo{person}{Augustin
  Chaintreau}.} \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{Seeding Network Influence in Biased Networks and
  the Benefits of Diversity}.
\newblock WWW'20.
\newblock


\bibitem[\protect\citeauthoryear{Stoica, Riederer, and Chaintreau}{Stoica
  et~al\mbox{.}}{2018}]%
        {StoicaRC18}
\bibfield{author}{\bibinfo{person}{Ana-Andreea Stoica},
  \bibinfo{person}{Christopher Riederer}, {and} \bibinfo{person}{Augustin
  Chaintreau}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Algorithmic Glass Ceiling in Social Networks}. WWW'18.
\newblock


\bibitem[\protect\citeauthoryear{Sunstein}{Sunstein}{2002}]%
        {Sunstein02}
\bibfield{author}{\bibinfo{person}{Cass~R. Sunstein}.}
  \bibinfo{year}{2002}\natexlab{}.
\newblock \showarticletitle{The Law of Group Polarization}.
\newblock \bibinfo{journal}{\emph{J. Political Philosophy}}
  \bibinfo{volume}{10}, \bibinfo{number}{2} (\bibinfo{year}{2002}),
  \bibinfo{pages}{175--195}.
\newblock


\bibitem[\protect\citeauthoryear{Tong, Prakash, Eliassi-Rad, Faloutsos, and
  Faloutsos}{Tong et~al\mbox{.}}{2012}]%
        {tong2012gelling}
\bibfield{author}{\bibinfo{person}{Hanghang Tong}, \bibinfo{person}{B~Aditya
  Prakash}, \bibinfo{person}{Tina Eliassi-Rad}, \bibinfo{person}{Michalis
  Faloutsos}, {and} \bibinfo{person}{Christos Faloutsos}.}
  \bibinfo{year}{2012}\natexlab{}.
\newblock \showarticletitle{Gelling, and melting, large graphs by edge
  manipulation}. CIKM'12.
\newblock


\bibitem[\protect\citeauthoryear{W{\k{a}}s, Waniek, Rahwan, and
  Michalak}{W{\k{a}}s et~al\mbox{.}}{2020}]%
        {wkas2020manipulability}
\bibfield{author}{\bibinfo{person}{Tomasz W{\k{a}}s}, \bibinfo{person}{Marcin
  Waniek}, \bibinfo{person}{Talal Rahwan}, {and} \bibinfo{person}{Tomasz
  Michalak}.} \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{The Manipulability of Centrality Measures-An
  Axiomatic Approach}. In \bibinfo{booktitle}{\emph{Proceedings of the 19th
  International Conference on Autonomous Agents and MultiAgent Systems}}.
  \bibinfo{pages}{1467--1475}.
\newblock


\bibitem[\protect\citeauthoryear{White and Smyth}{White and Smyth}{2003}]%
        {rwclosenessWhiteSmyth}
\bibfield{author}{\bibinfo{person}{Scott White} {and} \bibinfo{person}{Padhraic
  Smyth}.} \bibinfo{year}{2003}\natexlab{}.
\newblock \showarticletitle{Algorithms for Estimating Relative Importance in
  Networks}. KDD;03.
\newblock


\bibitem[\protect\citeauthoryear{Zeng, L{\"u}, and Zhou}{Zeng
  et~al\mbox{.}}{2012}]%
        {zeng2012manipulating}
\bibfield{author}{\bibinfo{person}{An Zeng}, \bibinfo{person}{Linyuan L{\"u}},
  {and} \bibinfo{person}{Tao Zhou}.} \bibinfo{year}{2012}\natexlab{}.
\newblock \showarticletitle{Manipulating directed networks for better
  synchronization}.
\newblock \bibinfo{journal}{\emph{New Journal of Physics}}
  \bibinfo{volume}{14}, \bibinfo{number}{8} (\bibinfo{year}{2012}),
  \bibinfo{pages}{083006}.
\newblock


\end{thebibliography}

